Analyzing Offline Social Engagements: An Empirical Study of Meetup Events Related to Software Development

Software developers use a variety of social media channels and tools in order to keep themselves up to date, collaborate with other developers, and find projects to contribute to. Meetup is one of such social media used by software developers to organize community gatherings. Liu et al. characterized Meetup as an event-based social network (EBSN) which contains valuable offline social interactions in addition to online interactions. Recently, Storey et al. found out that Meetup was one of the social channels used by developers. We in this work investigate in detail the dynamics of Meetup groups and events related to software development, which has not been done in any of the previous works. First, we identified 6,317 Meetup groups related to software development and extracted 185,758 events organized by them. Then we took a statistically significant sample of 452 events on which we performed open coding, based on which we were able to develop 9 categories of events (8 main categories + Others). Next, we did a popularity analysis of the categories of events and found that Talks by Domain Experts, Hands-on Sessions, and Open Discussions are the most popular categories of events organized by Meetup groups related to software development. Our findings show that more popular categories are those where developers can learn and gain knowledge. On doing a diversity analysis of Meetup groups we found 19.82% of the members on an average are female, which is a larger proportion as compared to numbers reported in previous studies on other social media. From a broader software development community point of view information from this new forum can be valuable to identify and understand emerging topics and associations among them which can be helpful to identify future trends as well as current best practices.

==> Discussion.tex <==
From our findings presented in Figure~\ref{fig:RQ2},  we can clearly see that the most popular category of events is \textit{Talks by Domain Experts}, followed by \textit{Hands-on Sessions} and { \em Open Discussions}. In events belonging to  these categories, participants get to know and use new things which they may not have active access to in their day job.  The popularity of these categories highlight the importance software developers give to continual learning. Also in such events the speakers or domain experts get to share their experience as well as showcase their knowledge. This certainly helps to advertise their skills and experience and build up a reputation in their community. Also from Figure~\ref{fig:RQ2b}, it can be observed that the interest in the events related to category \textit{Hands-on Sessions}  is very high. One reason for this phenomena is that in  \textit{Hands-on Sessions} participants actually work on exercises and modules, and thus have better understanding of the topic that is being discussed in the event. Also such events are more interactive and helps participants to learn from one another as well as domain experts who are conducting the sessions.  

%The next two popular categories are \textit{Social Events} and \textit{Conferences} which seem to support the need of developers to connect with other developers. The need to connect with other developers has also been highlighted in previous studies such as ~\cite{storey2017social,SingerFS14,treude2012programming}. The other categories such as \textit{Competitions} and {\em Job fairs} do not seem to be very popular among developers. It may be because for finding jobs developers may be using other mediums such as job sites and job consultancies. The less popularity of {\em Competitive} events such as {\em Hackathons} may be due to the effort and resources required to organize them. The effort required in attending events such as \textit{Talks by Domain Experts} is certainly less as one can just listen to the speaker and then walk away with something new. 


%From our findings presented in Section~\ref{sec.results},  we can clearly see that the most popular category of events is \textit{Talks by Domain Experts}, followed by category \textit{Hands-on Sessions} and { \em Open Discussions}. In events belonging to  these categories, participants get to know and use new things which they may not have active access to in their day job.  The popularity of these categories highlight the importance software developers give to continual learning. Also in such events the speakers or domain experts get to share their experience as well as showcase their knowledge. This certainly help to advertise their skills and experience and build up a reputation in their community. 


%However, from Figure~\ref{fig:RQ2b} it can be observed that the attendance in the events related to category \textit{Hands-on Sessions} is lower than { \em Open Discussions} and even  \textit{Social Events}. One reason for this phenomena can be the fact that most events of category  \textit{Hands-on Sessions} require participants to being their own device. Also many of them are workshops held by domain experts, and fees may be charged to attend such events.



%ate. % The high popularity of this category in line with the findings of Storey et al~\cite{storey2017social}, where they found that events and Meetups are used by developers for keeping up to date, support learning and displaying skills. 


%Also such events attract less participants as seen in Figure~\ref{fig:RQ2b} which may be due to the  time commitment required on  their part to find teams and actually hack together a usable software product in a few days.In events such as {\em Hackathons} much more dedication and  focus is required for an extended amount of time.
%The next two popular categories are \textit{Social Events} and \textit{Conferences} which seem to support the need of developers to connect with other developers. The need to connect with other developers has also been highlighted in previous studies such as ~\cite{storey2017social,SingerFS14,treude2012programming}. The other categories such as \textit{Competitions} and {\em Job fairs} do not seem to be very popular among developers. It may be because for finding jobs developers may be using other mediums such as job sites and job consultancies. The less popularity of {\em Competitive} events such as {\em Hackathons} may be due to the effort and resources required to organize them. The effort required in attending events such as \textit{Talks by Domain Experts} is certainly less as one can just listen to the speaker and then walk away with something new. 

A common theme across most event categories (except \textit{Social Events and Job Fairs}) is that by participating in such events developers gain knowledge based on experiences of another developers. The learning experienced  by developers in such settings may be different from what they learn through other channels. As compared to other channels the opportunity to physically interact with the presenters and other developers surely helps people to clarify any doubts fast. Also for the presenters at such events, they are able to get an immediate feedback and alternate perspectives on the work presented. The implications related to above observations above can be for the field of software engineering education research. Detailed insights gathered from data related to organization and participation information of popular events, can be used to understand what helps developers the most. Universities and any other organizations related to software engineering education, can use the results of such research in order to make their software engineering education programs more interactive and collaborative, hence increasing their effectiveness
 

%The advantages of acquiring knowledge from such events and the challenges faced in doing so can be a topic for further investigation. 

%The documentation of knowledge captured in such events can also be an area to looked into.
% Such knowledge can also be gained through other media such as blogs, screen casts etc., but the events organized using Meetup groups are different as they encourage physical  interaction among developers.

%Also a number of groups have started to come up where there is a focus in collaborative engagement which tend to organize more events related to category \textit{Hands-on Sessions},   as compared to traditional groups where the focus is more on events related to category {\em Talks by Domain Experts}.

We also did some gender analysis on group members and found that female representation in the Meetup groups being 19.82\% which is higher than what has been reported for other social channels,3-9\% on Github~\cite{vasilescu2015gender,david2008community} and 7\% on Stack Overflow~\cite{vasilescu2013gender}. This result has an implication for empirical software engineering researchers to dig deep into understanding what factors contribute to higher participation, and if those factors can be replicated elsewhere to improve female participation.  We were also able to find empirical evidence that average female participation in groups is higher if the group organizer is female. This servers as a cue for various communities such as open source organizations, software development companies etc. to increase the proportion of females in leadership roles in order to encourage more female participation in their organizations.



Based on the analysis of topic popularity, it can be observed that topics related to broad themes of {\em blockchain, machine learning, cross-platform development} etc. are becoming popular over last few years. An implication for software engineering researchers is to pursue more research into the software engineering challenges related to above fields. There already has been some inital traction in this area~\cite{tian2018deeptest,khomh2018software,semla19}. The automated or manual analysis of discussion and events in relevant Meetup groups can help software researchers to understand paint points faces by machine learning developers and data scientists. This can be good direction to bridge gap between academia and industry for solving issues related to software engineering for machine learning. Another implication can be increased focus on  the reasons for rise of cross-platform development technologies likes {\em kotlin and react-native} does deserve some more attention.  Some work has already begun in this area~\cite{mateus2018empirical,mateus2019adoption}. For future work, the data from Meetup events can be valuable for both software researchers and practitioners to understand  the best practices are employed by these new rising technologies, which can be then adopted in similar domains related to software development. Also some topics such as {\em mapreduce}, and {\em meteor} have been loosing popularity in last few years. Results from research  into understanding why these technologies are loosing popularity, can discover valuable insights for both software researchers and practitioners.


==> ExpAnalysis.tex <==
\as{Check If it needs to be removed}

Some basic statistics about our data set are also shown In Figure~\ref{fig:datastats} 
 \input{datastatstable}

==> RQ2old.tex <==
\subsection{RQ2. How do project topics change over time?}

For answering this research question, we measure impact metric for each topic in our dataset. Based on the value of this metric, we then determine whether a topic is increasing or decreasing in trend. A topic is considered to be increasing in trend if the difference between the impact metrics~\ref{sec:analysis} at the last time period (i.e., 2016) and the first time period (i.e 2008) is greater than zero. Likewise, a topic is considered to be decreasing if the same difference is lower than zero. Based on the difference in the impact score, we identify the top 5 topics with increasing and decreasing trends. We plot the increasing and decreasing trends for the top-5 topics in Figure~\ref{fig:RQ2I} and ~\ref{fig:RQ2D}, respectively.

%To decide the top 5 increasing and decreasing trends, we measure the %percentage changes between the impact score between the first  time period %and and current time period of a particular topics. We then plot this %increasing and decreasing trend for the top-5 topics having the largest %such differences as shown in  and, respectively.

 Topics that are increasing in popularity are generally about web front end and user interface while topics that are decreasing in popularity are mostly about backend programming. Interestingly, topics such as {\em Blogging Library}, {\em Content Management}, and {\em Image Viewers} are getting more popular. This may suggests that common users are starting to get familiar and comfortable in developing and managing their own website, which may explain the popularity increase of those topics.

\begin{figure}[htpb]
	\begin{center}
		\includegraphics[width=3.5in,height=3in]{res/RQ2I.png}
	\end{center}
	\caption{Top 5 Topics with Increasing Popularity}
	\label{fig:RQ2I}
\end{figure}



\begin{figure}[htpb]
	\begin{center}
		\includegraphics[width=3.5in,height=3in]{res/RQ2D1.png}
	\end{center}
	\caption{Top 5 Topics with Decreasing Popularity}
	\label{fig:RQ2D}
\end{figure}


==> RQ4New.tex <==
...
%%Among categories marked by $S$ in Table~\ref{tab.topics}, some {\em fully match} categories in GitHub {\em showcases}. These include: {\em Music}\footnote{See \url{https://github.com/showcases/music}}, {\em Web Frameworks}\footnote{{\em Web Application Frameworks} in GitHub -- see \url{https://github.com/showcases/web-application-frameworks}, {\em Operating Systems}\footnote{{\em Open Source Operating Systems} in GitHub -- see \url{https://github.com/showcases/open-source-operating-systems}}, {\em Text Editors}\footnote{See \url{https://github.com/showcases/text-editors}}, and {\em Security}\footnote{See \url{https://github.com/showcases/security}}.
%
%We check if our approach can identify additional projects belonging to the above-mentioned five categories, and find that we indeed can find additional projects. The list of additional projects for each of the five categories are shown in Table~\ref{tab:additional projects}.
%
%
%
%\begin{table}[!htb]
%	\caption{Sample Additional Projects Discovered}
%	\label{tab:additional projects}
%	\centering
%	\begin{tabular}{|l|}
%        \hline  {\em Category: Music}\\
%		\hline  https://github.com/SmartThingsUle/DLNA-PLAYER\\
%		  https://github.com/benkaiser/stretto\\
%		  https://github.com/revolunet/VLCcontrols\\
%		  https://github.com/eddturtle/TurtlePlayer\\
%		  https://github.com/yoichitgy/EECircularMusicPlayerControl\\
%        \hline  {\em Category: Web Frameworks}\\
%        \hline  https://github.com/nephila/djangocms-blog\\
%		  https://github.com/chaijs/chai\\
%		  https://github.com/grommet/grommet\\
%		  https://github.com/erik5388/jquery.gracket.js\\
%		  https://github.com/Cmdv/React-RxJS\\
%        \hline  {\em Category: Operating Systems}\\
%		\hline  https://github.com/SharpCoder/rpi-kernel\\
%		  https://github.com/pguyot/Einstein\\
%		  https://github.com/krinkinmu/aufs\\
%		  https://github.com/tornewuff/pycorn\\
%		  https://github.com/mbaltaks/doublecommand\\
%        \hline  {\em Category: Text Editors}\\
%		\hline  https://github.com/jclement/SublimePandoc\\
%		  https://github.com/dhategan/brackets-grunt\\
%		  https://github.com/mgussekloo/Tabright\\
%		  https://github.com/kimpettersen/random-sublime-text-plugin\\
%		  https://github.com/chuyik/brackets-snippets\\
%        \hline  {\em Category: Security}\\
%		\hline  https://github.com/xyproto/permissions2\\
%		  https://github.com/peredurabefrog/phpSecureLogin\\
%		  https://github.com/benbahrenburg/Securely\\
%		  https://github.com/robregonm/yii2-auth\\
%		  https://github.com/ahoward/middleman-gibberish\\
%        \hline
%	\end{tabular}\vspace{-0.05cm}
%\end{table}
%
%
%
%%\url{https://github.com/jclement/SublimePandoc \\
%%	    & https://github.com/kimpettersen/random-sublime-text-plugin \\
%%	    & https://github.com/gamebooster/dota2-lua-engine \\
%%	      4&https://github.com/bhauman/dotsters \\
%%	      5&https://github.com/lukapusic/soundcloud-dl\\
%%	      6&https://github.com/nltk/nltk\\
%%	      7&https://github.com/openai/gym\\
%%	      8& https://github.com/binarylogic/authlogic\\
%%	      9&https://github.com/composer/composer\\
%%	      10&https://github.com/Kitware/VTK\\	
%%	      \hline
%		%\textbf{Total}	   &246    &2324   \\
%		%\hline
%
%%As shown in Table~\ref{sec.res.rq3.te} we can see that our approach is able to detect some new projects related to existing projects in Github {\em showcases}. Projects 1 and 2 are plugins related to {\em Sublime Text} a popular code editor. Project 3 provides a scripting engine for Lua language with respect to {\em Dota} a popular Game. Project 4 is a game implemented in Clojure Script. Project 5 is a {\em Unix} based {\em Music} tool which can be used to download songs from online streaming websites such as {\em Soundcloud}. Project 6 and 7 are popular {\em Machine Learning} toolkits, where 6 is used for {\em Natural Language Processing} tasks whereas 7 is used for {\em Reinforcement Learning} related tasks. Project 9 is an example of {\em Productivty Tool} category and is used for dependency management of GitHub project. Project 10 is a visualization toolkit and can be considered in the {\em Data Visualization} category. Thus, the results above show the promise of our approach in discovering projects related to existing categories. 

==> RQ4_bkp.tex <==
%We attempt to analyze technology associations in the dataset using group topics (represented by {\em urlkey}). We believe that such analysis will be useful to gain some understanding of the technological landscape of software development-related Meetup groups. Similar analysis have previously been done for example on Stack Overflow~\cite{chen2016mining}. To discover network of topic co-occurrences, we applied frequent itemset mining, with the result for minimum support of 0.05 shown in Figure~\ref{fig:group-topic-cooccurrence005}. 

%We attempt to analyze topic associations for group topics in the dataset. We believe that such analysis will be useful to gain some understanding of the sets of topics that are often discussed or studied together in software development-related Meetup groups. %Similar analysis has previously been done on Stack Overflow~\cite{chen2016mining}.
%To discover network of topic co-occurrences, we applied association rule mining~\cite{agrawal1994fast} on the topics of the groups, with each group treated as a transaction and each topic as an item. During this process, we first find the sets of topics whose ratio of co-occurrence compared to total number of groups (i.e. support) exceed certain minimum support value {\em minsup}. We exclude {\em softwaredev} since it exists in all groups. Subsequently we mine association rules in form of $topic_1 \implies topic_2$ that meets or exceeds certain confidence threshold {\em minconf}, where {\em confidence} being the percentage of groups having both $topic_1$ and $topic_2$ compared to groups having $topic_1$. For each rule, we also compute the {\em lift}, which is the ratio of confidence of the rule to the expected confidence given the dataset, and use it to filter the rules that are potentially most useful (i.e. having high lift). Afterwards, we generate a graph with each topic in the final set of rules being represented as a node, and rules $topic_1 \implies topic_2$ being represented as edge between $topic_1$ to $topic_2$. The result is shown in Figure~\ref{fig:group-topic-cooccurrence}. The figure has also been shared at link\footnote{\url{https://goo.gl/oaA1gK}} for better visibility.

We attempt to analyze associations for topics related to groups in our dataset to see if we can find some interesting associations based on these topics. To discover network of topic co-occurrences, we applied association rule mining~\cite{agrawal1994fast} on the topics of the groups, with each group treated as a transaction and each topic as an item. %We used a process similar to what has been done in~\cite{chen2016mining}. 
During this process, we first find the sets of topics whose ratio of co-occurrence compared to total number of groups (i.e. support) exceed certain minimum support value {\em minsup}. We exclude {\em softwaredev} since it exists in all groups. Subsequently we mine association rules in form of $topic_1 \implies topic_2$ that meets or exceeds certain confidence threshold {\em minconf}, where {\em confidence} being the percentage of groups having both $topic_1$ and $topic_2$ compared to groups having $topic_1$. For each rule, we also compute the {\em lift}, which is the ratio of confidence of the rule to the expected confidence given the dataset, and use it to filter the rules that are potentially most useful (i.e.,having high lift). Afterwards, we generate a graph with each topic in the final set of rules being represented as a node, and rules $topic_1 \implies topic_2$ being represented as edge between $topic_1$ to $topic_2$. The result is shown in Figure~\ref{fig:group-topic-cooccurrence}. The figure has also been shared at url\footnote{\url{https://goo.gl/oaA1gK}} for better visibility.



We observed that in addition to natural association between, for example, programming language and library/framework written in that language (e.g. {\em dotnet} with {\em csharp} and {\em asp-net-mvc}), there are group topics such as {\em scrum} that are associated with other more abstract topics instead of specific software tools. We also observe cluster comprising mix of specific technologies and more abstract topics, such as {\em docker} with {\em devops} and {\em cloud-computing}. We believe that identification of such clusters may help someone who is new to a subfield of software development (e.g. cloud computing) to identify relevant tools for their work.



%We observed that the distribution of topics within Meetup groups related to software development is very uneven, with only 11 topics out of 3,282 are associated with more than 1000 groups, 121 topics associated with 100 groups or more, and 1,455 topics associated with only one group. Based on manual inspection, it appears that this is partly caused by variation of topics used for same concept, in addition to diversity of terms in the software development field itself. For example, there are separate topics for ``UI Design'' (with \em{urlkey} \em{ui-design}), ``UI/UX design'' (with \em{urlkey} \em{ui-ux-design}), ``UI/UX'' (with \em{urlkey} \em{ui-ux}) and ``UX/UI'' (with \em{urlkey} \em{ux-ui}). This affected our attempt to discover associations between technologies, and more importantly, will also be detrimental to attempts to match Meetup member interests with groups. Given this, there appears to be opportunity for application of automatic merging / aggregation of similar topics to Meetup groups. The most frequently-used topics are shown in Table~\ref{tab.tbl_topic}. 

%\begin{table}
%	\caption{Top 10 most commonly used topic, excluding {\em softwaredev} which is present in all groups}
%	
%	\label{tab.tbl_topic}
%	
%	\begin{tabular}{l|r}
%		\hline
%		\multicolumn{1}{c|}{\textbf{Topic}} & \multicolumn{1}{|c}{\textbf{Groups}} \\ 
%		\hline
%		computer-programming & 3842 \\
%		web-development & 3248 \\
%		opensource & 2508 \\
%		web & 2190 \\
%		newtech & 2153 \\
%		mobile-development & 1622 \\
%		javascript & 1332 \\
%		webdesign & 1279 \\
%		technology & 1158 \\
%		mobile-technology & 1058 \\
%		\hline 
%	\end{tabular} 
%\end{table}

\begin{figure}
	\centering
	%\includegraphics[width=1\linewidth]{res/gephi-ARM_minsup_0005_minconf_075_minlift_5}
	\includegraphics[width=1\linewidth]{res/topic_associations_new}
	\caption{Network of topic co-occurrence, at minimum support = 0.005, minimum confidence = 0.75, and minimum lift = 5. }
	\label{fig:group-topic-cooccurrence}
	
\end{figure} 
%\vspace{-0.5cm}
%\begin{table}
%		\caption{Top 10 most commonly used topic}
%		
%	\label{tab.tbl_topic}
%	
%	\begin{tabular}{|l|l|r|}
%		\hline
%		\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{urlkey}} & \multicolumn{1}{|c|}{\textbf{Groups}} \\ 
%		\hline
%		Software Development & softwaredev & 6327 \\ 
%		Computer programming & computer-programming & 3842 \\
%		Web Development & web-development & 3248 \\
%		Open Source & opensource & 2508 \\
%		Web Technology & web & 2190 \\
%		New Technology & newtech & 2153 \\
%		Mobile Development & mobile-development & 1622 \\
%		JavaScript & javascript & 1332 \\
%		Web Design & webdesign & 1279 \\
%		Technology & technology & 1158 \\
%		\hline 
%	\end{tabular} 
%\end{table}

==> RQ5.tex <==
\begin{figure*}[h]
	\centering
	%\includegraphics[width=1\linewidth]{res/gephi-ARM_minsup_0005_minconf_075_minlift_5}
	\includegraphics[width=1\linewidth]{res/topic_associations_new}
	%\caption{Network of topic co-occurrence, at minimum support = 0.005, minimum confidence = 0.75, and minimum lift = 5. }
	\vspace{-0.1cm}
	\caption{Network of topic co-occurrence}%, at minimum support = 0.005, minimum confidence = 0.75, and minimum lift = 5. }
	\label{fig:group-topic-cooccurrence}
	
\end{figure*} 
%\vspace{-0.15cm}

We have analyzed associations for topics related to groups in our dataset to see if we can find some interesting associations based on these topics. To discover network of topic co-occurrences, we applied association rule mining~\cite{agrawal1994fast} on the topics of the groups, with each group treated as a transaction and each topic as an item. %We used a process similar to what has been done in~\cite{chen2016mining}. 
During this process, we first find the sets of topics whose ratio of co-occurrence compared to total number of groups (i.e. support) exceed certain minimum support value {\em minsup}. We exclude {\em softwaredev} since it exists in all groups. Subsequently we mine association rules in form of $topic_1 \implies topic_2$ that meets or exceeds certain confidence threshold {\em minconf}, where {\em confidence} being the percentage of groups having both $topic_1$ and $topic_2$ compared to groups having $topic_1$. For each rule, we also compute the {\em lift}, which is the ratio of confidence of the rule to the expected confidence given the dataset, and use it to filter the rules that are potentially most useful (i.e.,having high lift). Afterwards, we generate a graph with each topic in the final set of rules being represented as a node, and rules $topic_1 \implies topic_2$ being represented as edge between $topic_1$ to $topic_2$. The result is shown in Figure~\ref{fig:group-topic-cooccurrence} at minimum support = 0.005, minimum confidence
= 0.75, and minimum lift = 5. The figure has also been shared at \url{http://tiny.cc/vdqdbz} for better visibility.

%The figure has also been shared at \url{https://goo.gl/oaA1gK} for better visibility.




We observed that in addition to natural association between, for example, programming language and library/framework written in that language (e.g. {\em dotnet} with {\em csharp} and {\em asp-net-mvc}), there are topical clusters of concepts such as ``{\em agile, scrum}'',  etc. that are associated with management of software development. Some of the clusters contain topics such as  ``{\em women-programmers, woman-software-developers}'' which point to the effort the software community is making in addressing diversity issues by organizing events focused on certain under represented sections. We also observe clusters comprising  of a mix of specific technologies, such as {\em docker} with {\em devops} and {\em cloud-computing}. This highlights technologies that are closely relevant to one another; and one may want to acquire expertise in these technologies together.%We believe that identification of such clusters may help someone who is new to a subfield of software development (e.g. cloud computing) to identify relevant tools for their work.


%We observed that in addition to natural association between, for example, programming language and library/framework written in that language (e.g. {\em dotnet} with {\em csharp} and {\em asp-net-mvc}), there are group topics such as {\em scrum} that are associated with other more abstract topics instead of specific software tools. We also observe cluster comprising mix of specific technologies and more abstract topics, such as {\em docker} with {\em devops} and {\em cloud-computing}. We believe that identification of such clusters may help someone who is new to a subfield of software development (e.g. cloud computing) to identify relevant tools for their work.



%We observed that the distribution of topics within Meetup groups related to software development is very uneven, with only 11 topics out of 3,282 are associated with more than 1000 groups, 121 topics associated with 100 groups or more, and 1,455 topics associated with only one group. Based on manual inspection, it appears that this is partly caused by variation of topics used for same concept, in addition to diversity of terms in the software development field itself. For example, there are separate topics for ``UI Design'' (with \em{urlkey} \em{ui-design}), ``UI/UX design'' (with \em{urlkey} \em{ui-ux-design}), ``UI/UX'' (with \em{urlkey} \em{ui-ux}) and ``UX/UI'' (with \em{urlkey} \em{ux-ui}). This affected our attempt to discover associations between technologies, and more importantly, will also be detrimental to attempts to match Meetup member interests with groups. Given this, there appears to be opportunity for application of automatic merging / aggregation of similar topics to Meetup groups. The most frequently-used topics are shown in Table~\ref{tab.tbl_topic}. 

%\begin{table}
%	\caption{Top 10 most commonly used topic, excluding {\em softwaredev} which is present in all groups}
%	
%	\label{tab.tbl_topic}
%	
%	\begin{tabular}{l|r}
%		\hline
%		\multicolumn{1}{c|}{\textbf{Topic}} & \multicolumn{1}{|c}{\textbf{Groups}} \\ 
%		\hline
%		computer-programming & 3842 \\
%		web-development & 3248 \\
%		opensource & 2508 \\
%		web & 2190 \\
%		newtech & 2153 \\
%		mobile-development & 1622 \\
%		javascript & 1332 \\
%		webdesign & 1279 \\
%		technology & 1158 \\
%		mobile-technology & 1058 \\
%		\hline 
%	\end{tabular} 
%\end{table}
%\vspace{-0.2cm}




%\begin{figure}
%	\centering
%	%\includegraphics[width=1\linewidth]{res/gephi-ARM_minsup_0005_minconf_075_minlift_5}
%	\includegraphics[width=1\linewidth]{res/topic_associations_new}
%	%\caption{Network of topic co-occurrence, at minimum support = 0.005, minimum confidence = 0.75, and minimum lift = 5. }
%		\vspace{-0.1cm}
%		\caption{Network of topic co-occurrence}%, at minimum support = 0.005, minimum confidence = 0.75, and minimum lift = 5. }
%	\label{fig:group-topic-cooccurrence}
%	
%\end{figure} 
%\vspace{-0.15cm}
%\begin{table}
%		\caption{Top 10 most commonly used topic}
%		
%	\label{tab.tbl_topic}
%	
%	\begin{tabular}{|l|l|r|}
%		\hline
%		\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{urlkey}} & \multicolumn{1}{|c|}{\textbf{Groups}} \\ 
%		\hline
%		Software Development & softwaredev & 6327 \\ 
%		Computer programming & computer-programming & 3842 \\
%		Web Development & web-development & 3248 \\
%		Open Source & opensource & 2508 \\
%		Web Technology & web & 2190 \\
%		New Technology & newtech & 2153 \\
%		Mobile Development & mobile-development & 1622 \\
%		JavaScript & javascript & 1332 \\
%		Web Design & webdesign & 1279 \\
%		Technology & technology & 1158 \\
%		\hline 
%	\end{tabular} 
%\end{table}

%START
%We attempt to analyze technology associations in the dataset using group topics (represented by {\em urlkey}). We believe that such analysis will be useful to gain some understanding of the technological landscape of software development-related Meetup groups. Similar analysis have previously been done for example on Stack Overflow~\cite{chen2016mining}. To discover network of topic co-occurrences, we applied frequent itemset mining, with the result for minimum support of 0.05 shown in Figure~\ref{fig:group-topic-cooccurrence005}. 

%We attempt to analyze topic associations for group topics in the dataset. We believe that such analysis will be useful to gain some understanding of the sets of topics that are often discussed or studied together in software development-related Meetup groups. %Similar analysis has previously been done on Stack Overflow~\cite{chen2016mining}.
%To discover network of topic co-occurrences, we applied association rule mining~\cite{agrawal1994fast} on the topics of the groups, with each group treated as a transaction and each topic as an item. During this process, we first find the sets of topics whose ratio of co-occurrence compared to total number of groups (i.e. support) exceed certain minimum support value {\em minsup}. We exclude {\em softwaredev} since it exists in all groups. Subsequently we mine association rules in form of $topic_1 \implies topic_2$ that meets or exceeds certain confidence threshold {\em minconf}, where {\em confidence} being the percentage of groups having both $topic_1$ and $topic_2$ compared to groups having $topic_1$. For each rule, we also compute the {\em lift}, which is the ratio of confidence of the rule to the expected confidence given the dataset, and use it to filter the rules that are potentially most useful (i.e. having high lift). Afterwards, we generate a graph with each topic in the final set of rules being represented as a node, and rules $topic_1 \implies topic_2$ being represented as edge between $topic_1$ to $topic_2$. The result is shown in Figure~\ref{fig:group-topic-cooccurrence}. The figure has also been shared at link\footnote{\url{https://goo.gl/oaA1gK}} for better visibility.

==> contribution.tex <==
\hl{To the best of our knowledge this empirical study is the first of its kind to analyze in depth software related offline social interactions (in our case Meetup related software events). We have also to build a topic association graph based on the data extracted which helped us to find and highlight inter relationships between various topics.}


==> datapreprocessing.tex <==
%\vspace{0.3cm}
%As described in section~\ref{subsec.dataext}, the {\em readme} file contains most of the information which can be used to infer what is broadly the topic of the project. However, {\em readme} file of GitHub project many a times contains information about installation, usage, support, licensing etc.
%In this part, we use a combination of existing natural language processing (NLP) based text preprocessing techniques, with some heuristics to extract the most relevant text which can help in identifying the topic of the project. We then evaluate our data set on a sampled subset of 10,000 projects . The main steps in our approach are described below.

In this part, we use a combination of popular text preprocessing techniques and some heuristics to extract the most relevant text which can help in identifying the topic of a repository from its {\em readme} file. The main steps of the data processing process are described below.
%\vspace{0.3cm}
%{\em Splitting Document to Text Segments:}
Firstly as a {\em readme} file contains a number of paragraphs or segments all of which may not be very informative, we split the file into segments.
%We went through some randomly selected 30 projects to examine how the paragraphs are structured inside the {\em readme} files and if they follow a certain pattern .A {\em readme} file typically contains a number of headings. Under each heading, we have text segment typically consisting of one or a few paragraphs. Typically one of the text segments contains a text that clearly describes the purpose of the code in the repository, while the others provide additional details such as installation procedure, license information, etc. After going through about some 30 random projects, we observed that the text in {\ readme} file is generally separated by headers.
%Based on this observation,
We split a readme file into text segments based on the headings -- if a {\em readme} file has $n$ headings, we will have $n$ text segments. These text segments are then preprocessed and filtered in the next two steps
% We observed that in most of the {\em readme} files are preceded by an header and all the text in-between 2 headers forms a coherent paragraph in most of the cases. So based on this observation, for all the {\em readme} files of the 10,000 projects extracted in section~\ref{subsec.dataext}, we split them into paragraphs, by considering  all the text in between 2 successive headers as one paragraph. These paragraphs are then preprocessed and evaluated in the next 2 steps for their relevance in being a descriptive paragraph.
%\vspace{0.3cm}
%{\em Text Preprocessing:}
After we have the text segments, we perform standard text preprocessing  steps of {\em tokenization, stop word removal and stemming} on each of the segments.
%This step involves the following sub-steps:
%	\begin{enumerate}
%		\item {\em Tokenization:} In this step the text is broken into tokens where each token corresponds to a word that appears in the text.
%		\item {\em Stop Word Removal:} The common English stop words, such as ``is'', ``are'', etc, appear very often and thus may interfere with the topic generation when LDA is run. So we remove these words using a list of English stop words provided at~\url{http://www.ranks.nl/stopwords}. %\ty{Added} \dl{Please add the URL to the list}
%		\item {\em Stemming:} After removing the stop-words we reduce a word to its root form (e.g., ``writing'' and ``written'' are both reduced to ``write'') using a popular stemming algorithm, i.e., Porter stemmer~\cite{porter1980algorithm}
%	\end{enumerate}
%\vspace{0.3cm} 	
%{\em Descriptive  Paragraph Selection:}
%As described before many of the preprocessed paragraphs contain no information with regards to determining the topic of the project. So
%In this step we used a heuristic to identify the paragraph which is most likely to be descriptive of the functionality realized by the code in the repository. As described in section~\ref{subsec.dataext}, the homepage of each GitHub project contains a 1-2 line description of the project. For each {\em readme} file we do the tokenization, stop-word removal and stemming of this description. We then determine the most similar paragraph to the preprocessed description which is considered as the most relevant to project's description. The similarity between the preprocessed description and the respective paragraphs is calculated based on Vector Space Model (VSM) which is explained below.
%{\em  Text Segment Selection}:
Thirdly as all segments may not be descriptive, we used a heuristic to identify the segment which is  descriptive of the functionality realized by the code in the repository. We refer to this as the descriptive text segment. %As described in Section ~\ref{subsec.dataext}, the homepage of each GitHub project contains a 1-2 line short description of the project.
Each GitHub project contains a 1-2 line short description of the project, which we fetched in the {\em Data Extraction phase}. A text segment which is the most similar to this  short description is likely to be the descriptive segment. The similarity between the short description and a text segment is calculated based on Vector Space
Model (VSM). Next, we measure similarity between the description and paragraph by computing the {\em cosine similarity}~\cite{manning2008introduction}
% which is explained below.


%Using VSM, each document (in our case the description and the  paragraph being evaluated) is represented as a vector of %weights.

%Using VSM, each document (in our case the short description or a text segment) is represented as a vector of weights. Each weight in the vector corresponds to a word in a document and the value of weight is calculated using the standard TF-IDF weighting scheme~\cite{manning2008introduction}.
%The first step to convert a textual document into a vector of weights is text preprocessing which we have already performed as explained previously in {\em Text Preprocessing}.
%Next, we measure similarity between the description and paragraph by computing the {\em cosine similarity}~\cite{manning2008introduction} of their corresponding weight vectors. The cosine similarity of two vectors $v_1$ and $v_2$ can be computed as:

%\[
%\frac{v_1 \cdot v_2}{\| v_1 \|\| v_2 \|}
%\]

%\noindent In the above equation, $\cdot$ is the dot operation between vectors and $\| v_i \|$ is the magnitude of vector $v_i$.



%\vspace{0.3cm}  	
%{\em Evaluation:}


%\vspace{0.3cm}  

==> datastatstable.tex <==
%  \begin{table}[h]
%  	\caption{Filtered Data Statistics w.r.t Events}
%  	\label{tab.rq1}
%  	\centering
%  	\begin{tabular}{p{3cm}|p{3cm}}
%  		\hline\textbf{ Filtering Method} & \textbf{Group Count} \\
%  		\hline
%  		 All in Tech category	   &54,585      \\
%  		\textit{SOTagList} Heuristic & 53,862	     \\ 	
%  		$\geq$10 Members &    53,229 \\
%		$\geq$10 Events  & 	   16,858  \\
%		\textit{Software Development Tag} Heuristic
% 		\hline
%  		\textbf{Final filtered}	   &\textbf{16,730}      \\
%  					
%  		\hline
%  	\end{tabular}
%  	\label{subsec.rem.dataextr}
%  \end{table}
  
  
  \begin{figure*}[thb]
  	\begin{center}
  		\includegraphics[width=6.4in]{res/MeetupApproach2.png}
  	\end{center}
  	\caption{Filtered Data Statistics\as{Update if member data not analyzed}}
  	\label{fig:datastats}
  \end{figure*}

==> discuss.tex <==
%Our analysis provides some insights on what kind of projects OSS developers build. Looking at popular topics, web and mobile appears to be popular platforms. While {\em API} topic comes out to be the most popular, this does not come as a surprise as many applications are usually built upon some existing third party APIs. Many projects in GitHub are also about {\em Build Management}, {\em Programming Constructs}, {\em Operating System} and {\em File/Data Storage Libraries}. Security is also a popular concern, which is in line with other popular topics (i.e., web and mobile). Hacking, phishing, and other vulnerabilities are more common in mobile and web applications. Naturally, web and mobile application developers should take more precautions on providing better security. This is reflected by the fact that {\em User Authentication and Security} appears as one of the top topics.
 
%Increasing trends in topics such as {\em React Framework} and {\em Content Management} along with decreasing trends in {\em Django}, {\em Ruby Framework}, and {\em Servers/Networking} suggest that there is a gradual shift from server-side to client-side development. In other words, web development is becoming more at the client side rather than the server side. Proliferations of HTML5\footnote{\url{https://www.w3.org/TR/html5/}} in modern browsers accelerate this shift. HTML5 provides better client side application capability such as drawing animation and video rendering. Developing at client side also allows for better user experience as application is more responsive and calculations are rarely needed to be offloaded to the server side application, which is very dependent on network speed and latency. 


%When we investigate trends in popular programming languages such as JavaScript and Python, each language seems to have their own niche areas/topics where they are popular. JavaScript, which is the de facto language for client side web application, shows a trend in which React, a popular framework, is becoming more popular. To some extent, JavaScript contributes in driving the trend in web development. Python, on the other hand,  seems to be the preferred choice for file scripting purposes as can be seen by the popularity of the topic {\em File/Data}. Another trend that can be observed for Python language is that it seem be increasingly used in in data science areas which is evident from the steep increase of the topic {\em Data/Database/Data Analysis} for python.

%The above analysis suggests that practitioners currently exploring JavaScript frameworks may consider adopting React framework for their JavaScript development. Also for developers who are interested in moving to data science or those already practicing data science but want to explore a new platform may consider Python as the programming language to build their data science solutions.

==> expsetting.tex <==
The overall framework of our approach is illustrated in Figure~\ref{fig:system}. First, we extracted the data of any group related to software development from ~\url{Meetup}\footnote{https://www.meetup.com/}.  From these groups we took a random sample of the  events organized  by them, and then analyzed the same using grounded theory methodology~\cite{corbin1990grounded}. This step helped us to answer our first research question. We then performed an exploratory analysis on the data to answer our other research questions.  We describe the steps in detail below.
 
 
 
%The overall framework of our approach is illustrated in Figure~\ref{fig:system}. It takes as input a set of GitHub projects and output a set of categories in three main steps: data extraction, topic modelling, and manual analysis. The data extraction step recovers from the repositories texts that describe functionalities realized by code stored in them. The topic modeling step processes these functionality descriptive texts to generate a set of topics using LDA-GA proposed by Panichella et al.~\cite{panichella2013effectively}. Each topic generated by LDA-GA corresponds to a ranked list of words characterizing the topics. LDA-GA outputs also inform us which projects are associated to each of the topics. The manual analysis step converts these topics (i.e., ranked lists of words) into categories. We describe these three steps in the following subsections.

%\begin{figure}[!htb]
%	\vspace{-0.5cm}
%	\begin{center}
%		\includegraphics[width=3.4in]{res/MeetUpApproach.pdf}
%	\end{center}
%	\caption{Overall Framework}
%	\vspace{-0.5cm}
%	\label{fig:system}
%\end{figure}

%\begin{figure*}[thb]
%	\begin{center}
%		\includegraphics[width=6.4in]{res/MeetUpApproach2.png}
%	\end{center}
%	\caption{Overall Framework}
%	\label{fig:system}
%\end{figure*} 


%\subsection{Data Extraction}
%\textbf{Data Extraction}
%\textbf{\textit{Data Extraction : }}
\subsubsection{Data Extraction:}
\input{dataextraction}
\label{subsec.datapreprocessing}


\subsubsection{Open Coding: }
%\textbf{Open Coding } 
\input{OpenCoding}
\label{subsec.opencoding}


\input{Analysis}
\label{subsec.expanalysis}


%\subsubsection{Data Analysis}
%\input{analysis}
%\label{subsec.analysis}
%
%In this preliminary experiments, we investigate the potential of our proposed approach using 10,000 fairly popular GitHub projects. In GitHub, developers can star a project and starring serves two purposes: it acts as a bookmark for the developers to keep a track of projects they are interested in, and also acts as a way to communicate appreciation of a project they like~\cite{ghstars}. We used the GitHub search API\footnote{\url{https://developer.github.com/v3/search/}} to identify the projects that have more than 20 stars, which returned 244,419 such projects. We then took a random sample of 10,000 projects. This is a  statistically significant sample, considering a confidence level of 95\% and a confidence interval of 1\%. After we have identified the 10,000 projects, using GitHub API\footnote{\url{https://developer.github.com/v3//}}, we collected the metadata about these projects and also crawled their GitHub home pages.
%
%In the manual analysis step, the authors discussed together what label would be best to explain the topics. 
%The authors did not consider any particular dimensions such as language, platform, business domains etc. They only considered top words in LDA model as guidelines for labeling a topic along with projects that belong to the topic. LDA-GA returns 49 topics. A majority of the topics, 33 to be exact, can be labeled properly. We also merge some of these topics since they are closely related. We end up with a collection of 21 categories. 
%
%
%
%
%%As dataset for our study, we pick fairly popular projects on GitHub. %For this work, any project which had no less than 20 stars as of 22.09.2016, is considered as fairly popular.
%%Past studies have also used number of stars as a yardstick of popularity, e.g.,~\cite{ray2014large}.
%%\dl{Where do you get the GitHub data from? Is it from GHTorrent? How do you find the list of all projects and then filter those with 20 or more stars? The information is missing here.-- explained below}


==> manualanalysis.tex <==
This manual analysis step requires ...
%The output of the previous step is a set of topics along with a set of projects that belong to each topic. Each topic is represented by a ranked list of words that best represent it. Unfortunately, LDA does not output a good name for each topic. Moreover, the topics may not be ideal. Some topics may need to be merged, and some other topics do not correspond to a coherent concept and may need to be deleted.
%
%This manual analysis step requires a data analyst to perform three actions:
%
%\begin{itemize}
%\item  First, the data analyst needs to identify and delete incoherent topics. These topics may arise due to the imperfection of the data extraction or topic modeling step. The data extraction step may output a wrong text segment which describes other information instead of the functionality of the code implemented in a repository. GA may learn a semi-optimal number of topics. LDA may learn a poor topic.
%    
%\item Next, the data analyst needs to infer a good representative name for each topic. The data analyst can get a hint of a good name for a topic by looking into the top words outputted by LDA and the projects that are associated with the topic.
%
%\item Finally, the data analyst needs to merge closely related topics into higher level topics. Topics inferred by LDA can be at different levels of granularity, and a data analyst may need to manually merge them.
%\end{itemize}
%
%For categorization no particular dimensions or predefined categories  were considered. Any coherent topic that could be inferred based on the LDA top words was considered as a category.
%
%%LDA is not a perfect tool and thus some manual step is needed. We need to convert
%
%%topics are labeled manually. Two of the authors sat together and discussed what label would be best to explain the topics. Top-5 words in LDA model are used as guidelines for labeling the topics. Most of the topics – 38 topics to be exact – can be labeled properly. However, the remaining topics cannot be labeled into a single topic. We have also checked the projects that contain those topics and found that they cannot be categorized into one coherent topic. Since such topics cannot be labeled as one independent topic, we simply refer to them as Others.

==> related_work_ebsn.tex <==
Sander and Seminar personally attend about 40 social events in one of the first studies conducted on Meetup~\cite{sander2005associations}.  Liu et al. introduced the term event-based social network (EBSN)  to categorize online services such a Meetup, Eventbrite etc. in ~\cite{Liu11}. In their work they investigated the heterogeneous nature and diffusion patterns inherent  across EBSNs.  A lot of works have proposed  improved  event recommendation  techniques for recommending events in EBSNs ~\cite{macedo2015context,lu2016location,qiao122014event,liao2016whether,gao2016collaborative,qiao2014combining,pham2015general}.



The effect of offline gatherings such as Meetup on community participation and social capital contribution has been investigated in ~\cite{sessions2010offline,shen2015exodus,vaughn2015meetup}.  The factors which determine the success of a Meetup group have been analyzed in ~\cite{lai2014can,pramanik2016can}, and A predictive model of the Meetup group success was proposed in ~\cite{pramanik2016predicting}. 


==> related_work_mup.tex <==
Storey et al on their  survey found out that Meetup is one of the important channels used by developers for activities  such as learning, keeping up to date, discovering and connecting with other developers, displaying skills etc. 



==> related_work_socialemdia.tex <==
As emphasized in Storey et al. social media has revolutionized the way software development is done~\cite{storey2017social}.  In another work by them the investigate how usage of various social and communication channels effect software development~\cite{storey2017social}.  They surveyed developers about  how they use various tools such as social coding websites, question answering forums .mailing lists, micro-blogging services, chat etc.  and found out the challenges developers face in using these tools. The role of social networking in software development was also examined in ~\cite{begel2013social}.
 
 There have been many works  which have analyzed individual tools or channels.   Stack Overflow is one of the most popular forums thats has been analyzed by researchers in recent years. Jones et al. were one of the first to study conversations in developer communities~\cite{jones2009conversations}. Barua et al. applied LDA to discover topics and trends present in questions and answers on StackOverflow~\cite{barua2014developers}. They found that the topics range widely from jobs to version control systems to C\# syntax; questions in some topics lead to discussions in other topics; and the topics gaining the most popularity over time are web development, mobile applications, Git, and MySQL. Vasilescu et al. did an analysis on how the developers usage of Stack Overflow and GitHub is related~\cite{vasilescu2013stackoverflow}. Tag prediction for question in Stack Overflow also seems to be a popular area in software engineering research and many approaches have been proposed for solving this problem~\cite{wang2014entagrec,zhou2017scalable,cai2016greta}.  Recently Uddin et al. proposed methods to identify opinionated sentences from Stack Overflow data and then mine aspects from such sentences~\cite{uddin2017automatic,uddin2017opiner,uddin2017resolving}.  Beyer et al. did a quantitative analysis of android tags on Stack Overflow~\cite{beyer2016grouping}.  Various other  studies have been performed on Stack Overflow data such as ~\cite{linares2013exploratory,zagalsky2017r,linares2014api,correa2014chaff,calefato2015mining,gomez2013study}. Also Stack Overflow data has been used to build or propose various tool such as ~\cite{autocomment,treude2016augmenting,campbell2017nlp2code} etc.
 
 Another channel that has received a lot of attention in research lately is GitHub, a social coding website.  Thung et al.~\cite{thung2013network}  analyzed GitHub developer network to understand characteristics of influential projects and developers. An analysis of  C and C++ projects from GitHub  was done to understand the usage of asserts in ~\cite{CasalnuovoDOFR15}.   Vasilescu et al. collected thousands of projects from GitHub, in order to understand t relationship between context-switching and  productivity of developers~\cite{VasilescuBXCDDF16}.  There have been a number of other  empirical studies pn GitHub  to analyze the developer behavior  and practices  such as ~\cite{blincoeIST15,kalliamvakouICSE15,sheoran2014understanding,multitaskingICSE16}. There also have been studies investigating relationship between programming languages and code quality based on GitHub projects~\cite{ray2014large,KochharWL16}. %~\cite{GousiosPD14}

 
 Other channels such as microblogs and screencasts related to software development have also received considerable attention in recent years.  A number of researchers have analyzed microblogs posted in Twitter (aka tweets) or built tools to support developers to better use Twitter for their day-to-day work.  inger et al. surveyed 271 and interviewed 27 active developers on Github~\cite{SingerFS14}. They found that many developers are using Twitter to ``keep up with the fast-paced development landscape''. Bougie et al. analyzed 11,679 tweets posted by 68 developers from three open source projects~\cite{Bougie11}.  Wang et al. analyzed 568 tweets posted by developers from the Drupal open source project~\cite{Wang13}, and found that Drupal developers use Twitter to coordinate efforts, share knowledge, encourage potential contributors to join, etc. Tian et al. analyzed behaviours of software microbloggers on a large dataset that contains more than 13 million tweets posted by 42 thousand microbloggers~\cite{Tian14}. A number of other studies have also analyzed the content produced in Twitter o build tools for content analysis such as by software developers such as ~\cite{Tian12does,Tian14,prasetyo12,sharma2015nirmal,sharma2017harnessing}. These ten groups include commercial, news, tools and code, question and answer, events, personal, opinion, tips, job, and miscellaneous. The topics discussed on Twitter by end users of software, and the implications it can have for requirements engineering and software evolution has been explored in~\cite{guzman2016needle,williams2017mining}.  Macleod et al. did an analysis of how developers use screencasts to share and document software knowledge~\cite{macleod2015code,macleod2017documenting}. An analysis of user comments on coding video tutorials present on YouTube was performed in ~\cite{poche2017analyzing}. Lin et al. recently studied how developers use {\em slack} to help them in their software development activities~\cite{lin2016developers}. The developers' user of news aggregators such as \textit{Reddit} and \textit{HackerNews} has been explored in ~\cite{aniche2018modern}.
  
  %It has been do a wide variety of research, ranging from studies to understanding how certain programming constructs are used by the developers to studies exploring the team and diversity structures of various projects.
  %They find that asserts have a significant effect on software quality. Vasilescu et al. analyse a large-dataset of 246 projects to analyze the impact of Continuous Integration (CI) on quality and productivity~\cite{VasilescuYWDF15}. They find that projects using CI have more pull requests from core contributors and fewer rejections from external developers. Furthermore, using CI leads to finding more bugs. Gousios et al. analyze 291 projects from GitHub which are written in various different programming languages to understand the pull-based software development model~\cite{GousiosPD14}. The authors find that 60\% of the pull-request are processed in a day and only 14\% of the projects unders active development use pull-requests.
  %Kochhar et al. analyze 50,000 projects from GitHub to understand the prevalence of test cases in open-source projects and correlation between test cases and various project development characteristics such as lines of code, cyclomatic complexity, number of bugs and number of developers~\cite{KochharBLJ13,KochharBLJ13-qsic}.
  %GitHub has also been explored from a perspective of how test cases are used in open-source projects in ~\cite{KochharBLJ13,KochharBLJ13-qsic}. Thung et al.~\cite{thung2013network} had analyzed the network structure of GitHub developers to understand characteristics of influential projects and developers. Vasilescu et al. collect thousands of projects from GitHub to understand the rate and breadth of developers' context-switching behavior and the effect of context-switching on productivity~\cite{VasilescuBXCDDF16}. Different that the above studies, the goal of our work is to catalog Github repositories by expanding GitHub {\em showcases}.%The authors also survey developers to understand reasons for switching between projects. They find that biggest reason for multitasking is dependencies between projects and developers who work on many projects have higher productivity, if they work on few projects per day. Moreover, developers that switch too much during a day have lower productivity. In other work they use a mixed-methods approach and analyze a large number of projects from GitHub as well as survey thousands of developers to understand the impact of gender and tenure diversity of team productivity and turnover~\cite{VasilescuPRBSDF15}
  %Other channels such as microblogs and screencasts related to software development have also received considerable attention in recent years. There  have  been studies on how developers use microblogs and if information can be extracted easily from them~\cite{Storey2014,SingerFS14,Bougie11,Wang13,Tian14,Tian12does,prasetyo12,sharma2015nirmal,sharma2017harnessing,williams2017mining,el2017tweets}. Macleod et al. did an analysis of how developers use screencasts~\cite{macleod2015code,macleod2017documenting}. Ponzanelli et al. proposed an approach to extract relevant parts of the video automatically  in ~\cite{ponzanelli2016codetube,ponzanelli2017automatic}.
  
  % \as{add stuff from thesisi lit rev here}


==> related_work_socialemdia_short.tex <==
As emphasized by Storey et al., social media has revolutionized the way software development is done~\cite{storey2014r}.  In their recent work, Storey et al. have also investigated how usages of various social and communication channels affect software development~\cite{storey2017social}. % They surveyed developers about  how they use various tools such as social coding websites, question answering forums .mailing lists, micro-blogging services, chat etc.  and found out the challenges developers face in using these tools. 
The role of social networking in software development was also examined by several other prior works~\cite{begel2013social,storey2010impact}. There have been many works  which have analyzed individual sites or channels; we describe some of them below.

Stack Overflow is one of the most popular channels that has been a subject of many empirical studies~\cite{jones2009conversations,barua2014developers,vasilescu2013stackoverflow,linares2013exploratory,linares2014api,calefato2015mining}. Also, Stack Overflow data has been used to build various automated tools to support software development~\cite{treude2016augmenting,uddin2017automatic,tian2017apibot,murgia2016among,chen2016mining,baltes2018sotorrent}. Another channel that has received a lot of attention  is GitHub, a social coding website.  There have been various works studying developer behaviors and practices by analyzing data in GitHub~\cite{blincoeIST15,kalliamvakouICSE15,thung2013network,VasilescuBXCDDF16,CasalnuovoDOFR15,ray2014large,rastogi2016forking,rastogi2018relationship,baltes2019usage}. There have also been studies that investigate other channels such as Twitter and YouTube on contents related to software development. Developers' usage of  microblogs and ways to improve information extraction from microblogs have been explored by a number of prior studies~\cite{Storey2014,SingerFS14,Bougie11,Wang13,Tian14,sharma2015nirmal,sharma2017harnessing,el2017tweets}.  Analysis of how developers use screencasts was explored in ~\cite{macleod2015code}. Methods to extract relevant fragments from software development videos tutorials have been discussed in  ~\cite{ponzanelli2016codetube,ponzanelli2017automatic}.
%Macleod et al. did an analysis of how developers use screencasts~\cite{macleod2015code}. Ponzanelli et al. proposed an approach to extract relevant fragments from software development videos tutorials ~\cite{ponzanelli2016codetube,ponzanelli2017automatic}.




  %Jones et al. studied conversations in developer communities. Barua et al. applied LDA to discover topics and trends present in questions and answers on StackOverflow~\cite{barua2014developers}. %They found that the topics range widely from jobs to version control systems to C\# syntax; questions in some topics lead to discussions in other topics; and the topics gaining the most popularity over time are web development, mobile applications, Git, and MySQL. 
  %Vasilescu et al. did an analysis on how the developers usage of Stack Overflow and GitHub is related~\cite{vasilescu2013stackoverflow}. %Tag prediction for question in Stack Overflow also seems to be a popular area in software engineering research and many approaches have been proposed for solving this problem~\cite{wang2014entagrec,zhou2017scalable}.  
  %Recently Uddin et al. proposed methods to identify opinionated sentences from Stack %Overflow data and then mine aspects from such sentences~\cite{uddin2017resolving}.  Beyer et al. did a quantitative analysis of android tags on Stack Overflow~\cite{beyer2016grouping}.  
  %Various other  studies have been performed on Stack Overflow data to mine information related to software artifacts ~\cite{linares2014api,calefato2015mining,beyer2016grouping,uddin2017resolving}. 


%Thung et al.~\cite{thung2013network}  analyzed GitHub developer network to understand characteristics of influential projects and developers. An analysis of  C and C++ projects from GitHub  was done to understand the usage of asserts in ~\cite{CasalnuovoDOFR15}.   Vasilescu et al. collected thousands of projects from GitHub, in order to understand t relationship between context-switching and  productivity of developers~\cite{VasilescuBXCDDF16}.  There have been a number of other  empirical studies pn GitHub  to analyze the developer behavior  and practices  such as ~\cite{blincoeIST15,kalliamvakouICSE15}%sheoran2014understanding,multitaskingICSE16}. %There also have been studies investigating relationship between programming languages and code quality based on GitHub projects~\cite{ray2014large,KochharWL16}. %~\cite{GousiosPD14}


%It has been do a wide variety of research, ranging from studies to understanding how certain programming constructs are used by the developers to studies exploring the team and diversity structures of various projects.
%They find that asserts have a significant effect on software quality. Vasilescu et al. analyse a large-dataset of 246 projects to analyze the impact of Continuous Integration (CI) on quality and productivity~\cite{VasilescuYWDF15}. They find that projects using CI have more pull requests from core contributors and fewer rejections from external developers. Furthermore, using CI leads to finding more bugs. Gousios et al. analyze 291 projects from GitHub which are written in various different programming languages to understand the pull-based software development model~\cite{GousiosPD14}. The authors find that 60\% of the pull-request are processed in a day and only 14\% of the projects unders active development use pull-requests.
%Kochhar et al. analyze 50,000 projects from GitHub to understand the prevalence of test cases in open-source projects and correlation between test cases and various project development characteristics such as lines of code, cyclomatic complexity, number of bugs and number of developers~\cite{KochharBLJ13,KochharBLJ13-qsic}.
%GitHub has also been explored from a perspective of how test cases are used in open-source projects in ~\cite{KochharBLJ13,KochharBLJ13-qsic}. Thung et al.~\cite{thung2013network} had analyzed the network structure of GitHub developers to understand characteristics of influential projects and developers. Vasilescu et al. collect thousands of projects from GitHub to understand the rate and breadth of developers' context-switching behavior and the effect of context-switching on productivity~\cite{VasilescuBXCDDF16}. Different that the above studies, the goal of our work is to catalog Github repositories by expanding GitHub {\em showcases}.%The authors also survey developers to understand reasons for switching between projects. They find that biggest reason for multitasking is dependencies between projects and developers who work on many projects have higher productivity, if they work on few projects per day. Moreover, developers that switch too much during a day have lower productivity. In other work they use a mixed-methods approach and analyze a large number of projects from GitHub as well as survey thousands of developers to understand the impact of gender and tenure diversity of team productivity and turnover~\cite{VasilescuPRBSDF15}


%Other channels such as microblogs and screencasts related to software development have also received considerable attention in recent years. There  have  been studies on how developers use microblogs and if information can be extracted easily from them~\cite{Storey2014,SingerFS14,Bougie11,Wang13,Tian14,Tian12does,sharma2015nirmal,sharma2017harnessing,el2017tweets}. Macleod et al. did an analysis of how developers use screencasts~\cite{macleod2015code}. Ponzanelli et al. proposed an approach to extract relevant parts of the video automatically  in ~\cite{ponzanelli2016codetube,ponzanelli2017automatic}.



==> researchdata.tex <==
As dataset for our study, we pick fairly popular projects on GitHub. For this work, any project which had no less than 20 stars as of 22.09.2016, is considered as fairly popular. In GitHub, developers can star a project and starring serves two purposes: it acts as a bookmark for the developers to keep a track of projects they are interested in, and also acts as a way to communicate appreciation of a project they like~\cite{ghstars}. Past studies have also used number of stars as a yardstick of popularity, e.g.,~\cite{ray2014large}. \dl{Where do you get the GitHub data from? Is it from GHTorrent? How do you find the list of all projects and then filter those with 20 or more stars? The information is missing here.}

We find a total of 244,419 projects with 20 or more stars, out of which we then randomly sampled about 10,000 projects. This sample gives us a confidence interval of 95$^+_-$1 percent. We collected the meta-data about these 10,000 projects using GitHub API\footnote{\url{https://developer.github.com/v3//}} which provides information about various repositories and/or users present on GitHub. We also crawled the GitHub home pages of all these 10,000 projects to extract the text required for extracting topical information about these projects. The topic association of these 10,000 projects was then combined with their meta-data to perform our analysis. The details about the whole process are covered in Section~\ref{subsec.rem}.

%As described earlier GitHub is one of the most popular site for sharing code and coding projects. It allows developers and even firms to share there projects with other interested developers. Other developers can show their interest in a particular project by starring it. Starring a project serves two purposes, In our work, we use stars as a metric to  measure the popularity of GitHub projects. Such a methodology has also been used in previous work such as 





